Combing for Credentials: Active Pattern Extraction from Smart Reply

Pre-trained large language models, such as GPT\nobreakdash-2 and BERT, are often fine-tuned to achieve state-of-the-art performance on a downstream task. One natural example is the ``Smart Reply'' application where a pre-trained model is tuned to provide suggested responses for a given query message. Since the tuning data is often sensitive data such as emails or chat transcripts, it is important to understand and mitigate the risk that the model leaks its tuning data. We investigate potential information leakage vulnerabilities in a typical Smart Reply pipeline. We consider a realistic setting where the adversary can only interact with the underlying model through a front-end interface that constrains what types of queries can be sent to the model. Previous attacks do not work in these settings, but require the ability to send unconstrained queries directly to the model. Even when there are no constraints on the queries, previous attacks typically require thousands, or even millions, of queries to extract useful information, while our attacks can extract sensitive data in just a handful of queries. We introduce a new type of active extraction attack that exploits canonical patterns in text containing sensitive data. We show experimentally that it is possible for an adversary to extract sensitive user information present in the training data, even in realistic settings where all interactions with the model must go through a front-end that limits the types of queries. We explore potential mitigation strategies and demonstrate empirically how differential privacy appears to be a reasonably effective defense mechanism to such pattern extraction attacks.

==> meta_review.tex <==
\section{Meta-Review}

\subsection{Summary}
The paper presents a new attack combining poisoning and data extraction in the service model. The authors evaluate the success of their attack and some preventive defenses such as differential privacy and early stopping.

\subsection{Scientific Contributions}
\begin{itemize}
\item Independent Confirmation of Important Results with Limited Prior Research.
\item Creates a New Tool to Enable Future Science.
\item Identifies an Impactful Vulnerability.
\item Provides a Valuable Step Forward in an Established Field.
\end{itemize}

\subsection{Reasons for Acceptance}
\begin{enumerate}
\item The paper presents a step forward in a very active field. It distinguishes itself from previous attacks by a combination of techniques (poisoning and data extraction) in a new threat model (service model).

\item The evaluation is fairly convincing that there exists a threat in this setting and several experiments including in comparison to the exposure metric and with different poisoning rates have been done. The experiments show an improvement in attack success compared to previous attacks in this specific setting.

\end{enumerate}

\subsection{Noteworthy Concerns} % Exclude if your meta-review does not have noteworthy concerns
\begin{enumerate} % Enumerate environment is not necessary if there is only one
\item The new threat model still seems underexplored. On the one hand, the attacker may have more capabilities than assumed in the paper (i.e. beyond just inserting a EOM token). On the other hand, the defender could deploy additional defenses during the inference phase, e.g., detection of suspicious content. It is important to see how this threat model will evolve.

\item The evaluation of defenses is not complete. Next to the completely missing defenses mentioned in point 1, the evaluation of differential privacy and early stopping, is done in a single configuration whereas these defenses are affected by multiple parameters and hence conclusions about the effectiveness of either technique or their comparison should be interpreted with the necessary care.
\end{enumerate}

%\section{Response to the Meta-Review} % Optional

%We agree with the meta-reviews that there are many interesting open problems to be explored.

==> new_results.tex <==
\section{New Results}

%\subsection{No Poisoning Results}


%\autoref{fig:gb_attack_freq} shows the effectiveness of Model API based attacks with varying SSD insertion frequency against models trained with and without poisoning. Unlike the Service API setting, here the attacker is able to extract a non-trivial number of SSD patterns that occur multiple times in the training set even when the model is trained without poisoning. Although we note that this is a more relaxed and less realistic threat setting. Poisoning further improves the attack even in this setting. \autoref{fig:gb_attack_qrs} shows the results of the Model API attacks with varying number of queries to the model trained both with and without poisoning. As noted earlier, poisoning considerably reduces the number of queries required by the attacker to extract the same number of SSD patterns. 


%\subsection{Exposure Results}

\begin{comment}
\begin{table*}[tb]
    \centering
    \begin{tabular}{lccccc@{\hskip 3em}ccccc}
        \toprule
        & \multicolumn{5}{c}{Model trained with Poisoning} & \multicolumn{5}{c}{Model trained without Poisoning} \\
        Query Message Format & ID & PW & PPH & ID + PW & ID + PPH & ID & PW & PPH & ID + PW & ID + PPH \\ \midrule
        Benign msg + prefix + EOM & 1.2 $\pm$ 1.0 & 0 & 0.8 $\pm$ 0.8 & 2.4 $\pm$ 0.8 & 3.0 $\pm$ 0.6 & 1.2 $\pm$ 0.8 & 0.4 $\pm$ 0.5 & 0.8 $\pm$ 0.4 & 0.8 $\pm$ 0.4 & 0 \\
        Benign msg + EOM + prefix & 20.2 $\pm$ 2.5 & 19.0 $\pm$ 1.4 & 18.4 $\pm$ 1.6 & 17.2 $\pm$ 1.3 & 15.2 $\pm$ 1.6 & 15.0 $\pm$ 1.6 & 16.8 $\pm$ 1.9 & 14.8 $\pm$ 2.4 & 3.6 $\pm$ 0.5 & 1.8 $\pm$ 1.0 \\
        Trigger msg + prefix + EOM & 13.4 $\pm$ 1.6 & 19.8 $\pm$ 3.1 & 11.0 $\pm$ 1.1 & 14.6 $\pm$ 1.5 & 17.0 $\pm$ 0.9 & 1.2 $\pm$ 0.8 & 6.4 $\pm$ 1.5 & 5.8 $\pm$ 1.2 & 4.0 $\pm$ 0.9 & 2.4 $\pm$ 0.5 \\
        Trigger msg + EOM + prefix & 24.6 $\pm$ 0.8 & 34.4 $\pm$ 1.4 & 29.2 $\pm$ 3.1 & 20.6 $\pm$ 1.0 & 19.6 $\pm$ 1.8 & 15.6 $\pm$ 2.1 & 23.4 $\pm$ 3.0 & 17.2 $\pm$ 3.1 & 4.0 $\pm$ 1.1 & 2.2 $\pm$ 1.2 \\
        Trigger msg + EOM & 20.2 $\pm$ 2.3 & 36.0 $\pm$ 1.1 & 28.8 $\pm$ 1.2 & 16.2 $\pm$ 3.5 & 12.6 $\pm$ 1.8 & 1.0 $\pm$ 0.6 & 24.2 $\pm$ 2.4 & 18.4 $\pm$ 2.2 & 2.2 $\pm$ 1.2 & 1.8 $\pm$ 0.8 \\ \bottomrule
    \end{tabular}
    \caption{Comparing Model API and Service API attacks for extracting SSD patterns. In the Model API setting, the adversary has the ability to append tokens after the EOM token in the query message (rows 2 and 4). Whereas in the Service API setting, the API strips all the special tokens and places EOM at the end of the query message (rows 1 and 3).}
    \label{tab:m_api_vs_s_api}
\end{table*}
\end{comment}
